RT-DAP: A Real-Time Data Analytics Platform for Large-scale Industrial Process Monitoring and Control

In most process control systems nowadays, process measurements are periodically collected and archived in historians. Analytics applications process the data, and provide results offline or in a time period that is considerably slow in comparison to the performance of the manufacturing process. Along with the proliferation of Internet-of-Things (IoT) and the introduction of "pervasive sensors" technology in process industries, increasing number of sensors and actuators are installed in process plants for pervasive sensing and control, and the volume of produced process data is growing exponentially. To digest these data and meet the ever-growing requirements to increase production efficiency and improve product quality, there needs to be a way to both improve the performance of the analytics system and scale the system to closely monitor a much larger set of plant resources. In this paper, we present a real-time data analytics platform, called RT-DAP, to support large-scale continuous data analytics in process industries. RT-DAP is designed to be able to stream, store, process and visualize a large volume of realtime data flows collected from heterogeneous plant resources, and feedback to the control system and operators in a realtime manner. A prototype of the platform is implemented on Microsoft Azure. Our extensive experiments validate the design methodologies of RT-DAP and demonstrate its efficiency in both component and system levels.

==> abstract.tex <==
\section{abstract} \label{sec:abstract}

In most process monitoring and control systems nowadays, process measurements are periodically collected and archived in historians. Analytics applications read data from these historians, process the data, and provide results offline or in a time period that is considerably slow in comparison to the performance of the manufacturing process. Along with the proliferation of Industrial Internet-of-Things (IIoT), the volume
of produced process data is growing exponentially. To digest these data and meet the ever-growing requirements to increase production efficiency and improve product quality, there needs to be a way to both improve the performance of the analytics system and scale the system to closely monitor a much larger set of plant resources. In this paper, we present a scalable real-time data analytics platform to support large-scale continuous data analytics. The proposed platform will be able to stream, store, process and visualize a large volume of real-time data flows collected from heterogenous plant resources, and feedback to the system and operators in a real-time manner. We implement the platform on Microsoft Azure and our extensive experiments demonstrate the effectiveness of the proposed data analytics platform in providing real-time data streaming, storage, decision making and visualization.


==> case.tex <==
\section{Case Study} \label{sec:case}

In addition to evaluating the component- and system-level performance of the proposed data analytics platform using the real-time measurement data streamed from the Crude simulator, we further integrate the analytics platform with an operational chemical plant as a case study to demonstrate the efficiency of the platform for both offline and online analytics. The data for this case study was collected from the Divided Wall Column (DWC) at the J.J. Pickle Research Campus at the University of Texas at Austin~\cite{SRP}. An overview of the DWC (top) and its design and implementation details (bottom) are shown in Fig.~\ref{fig:dwc}. It is highly instrumented with both wired and wireless instrumentation.

The application of DWC distillation offers the potential of significant energy and capital savings by effectively combining two distillation columns into one~\cite{cep02}. The DWC contains a column, feed tank, reflux tank, feed preheater, reboiler and an overhead condenser. A section of the DWC contains an interior wall that separates the column into two sides.  The feed is sent to one side and a third product is removed on the opposite side of the wall. The DWC contains packed sections that are located at the very top and bottom of the column. In between the packed sections are two divided wall sections that have a feed section in-between.  The feed section is located on the 'A' side of the column and side product will be removed on the 'B' side.  The side product is split into two streams.  One stream is recycled back to the column while the other product is returned to the feed tank. The DWC is a multifunctional distillation column that can be operated in total reflux mode, total reflux with feed and product loops, and total reflux utilizing two column product streams.

Twenty-seven wireless devices are installed on the DWC. These devices measure flows, levels, pressures, temperatures, and valve positions. In this case study, we are separating three hydrocarbons: C5, C6, and C7. The flows for this separation are described on the left hand side of Fig.~\ref{fig:model}. Our objective is to estimate C5, C6, and C7 at each of the 5 locations (630, 640, Feed, Overhead, Bottoms). For this installation we are estimating 3 components at 5 locations, {\em i.e.} 15 inferred compositions. For each specific inferred composition measurement, For offline analytics, we can extract data in chunks from very specific sections in HBase and merge them for the modeling application. For continuous analytics, we will accumulate data from the real-time process measurements within a specified time window and execute the model periodically, and write the results back to into the control systems for the operators. The partial least squares (PLS) regression models for C7 estimation in both offline and online analytics are illustrated on the right side of Fig.~\ref{fig:model}.

\noindent {\bf 1) Need to provide more details of the DWC, including how many devices and their sampling rates in the experiments; 2) Describe how to perform the queries, through online streams or HBase records; 3) How to implement PLS on Storm and its benefits; 4) show the experimental results.}

\eat{We built an experimental testbed to prove the concept and validate our design. Our data sources include sensor measurements and network health messages collected from three WirelessHART networks. All collected data is streamed into a Kafka system which organizes all data tuples into prioritized queues. These data tuples are then consumed by the Storm cluster which distributes them in the Storm topology for real-time processing. The final results are stored in the HBase. The model editor retrieves and processes the data archived in HBase through the Thrift interface and adjusts the analytics models if necessary and feedback to the Storm topology. We also implemented a rich set of web services. This enables the users to visualize the real-time data streams in a friendly way and display network and device statistic information.}

\begin{figure}
   \centering
   \includegraphics[width=0.9\linewidth]{figs/dwc.pdf}
   \caption{\small An overview of the Divided Wall Column (DWC) and its design and implementation details}
   \label{fig:dwc}
\vspace{-0.2in}
\end{figure}

\eat{
\begin{figure*}
   \centering
   \includegraphics[width=1.0\linewidth]{figs/setup.pdf}
   \caption{\small Wireless instrumentation of the Divided Wall Column and three test settings on packet capture and analytics}
   \label{fig:dwc}
\end{figure*}}

\begin{figure*}
   \centering
   \includegraphics[width=1.0\linewidth]{figs/PLS-model.pdf}
   \caption{\small Offline and online partial least squares (PLS) regression modeling for C7 estimation}
   \label{fig:model}
\end{figure*}


==> design-naming.tex <==
\subsection{Preliminaries} \label{sec:design:preliminaries}
We are using the following naming convention to define the tags in the network health analytics project. 

For each kind of time series data, we assign it a unique tag string for storing and retrieving purpose. 
The tag will be a combination of network location, Gateway Unique ID, Device Unique ID and the name of physical measurements or health information. 
The format can be represented by the following formula if it is a data directly from gateways or it shows in the following format if it is a data from devices.

\begin{center}
$NetworkLocation::GatewayUID/DeviceUID/Value$
\end{center}


The following is a tag of a gateway health information value. The location of the gateway is "UCONN-ITEB-311"; the gateway unique ID is "A5EF69D256" and "Health" means that the this tag represents the Health Information.

\begin{center}
UCONN-ITEB-311::A5EF69D256/Health
\end{center}

The following is a tag of a device health information value and a measurement value. The location of the gateway is "UCONN-ITEB-311"; the gateway unique ID is "A5EF69D256"; the device unique ID is "A286BD21FA"; "Health" means that this tag represents the Health Information and "OUT.PV" means that this tag represents the "PV" device value.

\begin{center}
UCONN-ITEB-311::A5EF69D256/A286BD21FA/Health              

UCONN-ITEB-311::A5EF69D256/A286BD21FA/OUT.PV               
\end{center}

==> design-visualization.tex <==
\subsection{Real-Time Data Visualization} \label{sec:design:visualization}

A user-friendly UI can greatly help the plant operator to closely monitor and diagnose various plant resources. To this end, we have developed a web server running on the portal VM with a rich set of web services. The web server connects to the HBase through Thrift interface, fetches the raw/aggregated measurement data and analytics results, and provides real-time data visualization at various time scales to both plant operators and authorized end users.

By using AJAX, the front end can be programmed easily. The webpage can be divided into multiple chart blocks. Each chart block works independently to display a chart and it can be added or removed by the end users. Within a chart block, the users can choose the time period and tags to display and compare with. The webpage accesses the Servlet API on the web server, which returns the dataset using XmlHttpRequest. Upon the receipt of the dataset, the webpage draws curve(s) in the corresponding chart block. After the initial curve(s) is drawn, the time period can be adjusted manually, or by using zooming and shifting functions. The tag list can also be adjusted in the runtime. Other built-in functions of the web interface include raw data file uploading/downloading, which allow the end users to upload or download datasets to and from the RTDB manually.

\eat{
\begin{figure}
\includegraphics[width=0.45\textwidth]{figs/visualization.pdf}
\caption{\footnotesize Web UI designed for real-time data visualization}
\label{fig:visualization}
\vspace{-0.1in}
\end{figure}

\vspace{0.05in}
\noindent {\bf The visualization figure should be replaced with a more representative one.}
\vspace{0.05in}}



==> related-bak.tex <==
\section{Related Works} \label{sec:related}

The Internet of Things (IoT) has drawn a tremendous amount of attention in recent years. A growing number of physical objects are connected to the Internet at an unprecedented rate~\cite{al2015internet}.
According to~\cite{IDCwhitepaper}, in 2011, the overall created and copied data volume in the world was 1.8ZB ($\approx 10^{21}$B), which increased by nearly nine times within five years~\cite{chen2014big}.
There have been 6 billion mobile subscriptions in the world and every day 10 billion text messages are sent. By the year 2020, 50 billion devices will be connected to networks and the internet and it is expected that total amount of data on earth will reach 35 ZB~\cite{zaslavsky2013sensing,gerhardt2012unlocking,sagiroglu2013big}. To make one step further utilizing the data, researchers has carried out a number of data analytics systems in different domains such as smart city and transportation ~\cite{dobre2014intelligent,fiosina2013big}, smart health care~\cite{gad2011cloud,doukas2011managing}.
In industrial, particularly for process control applications and industrial automation, companies are building comprehensive data analytic platforms and they also provide white paper describe briefly on the platforms.
In June 2013, HP announced the HAVEn platform for analyzing and finding meaning from big data. In January 2014, HP released a new version of HP IDOL that strengthens integration with several key components of the HAVEn platform by expanding upon IDOL’s analytics, reliability and ease of use~\cite{wiki:haven}. Hadoop and vertica are used in HP IDOL.
Intel also proposed its Industrial Solutions system consolidation series - a virtualized industrial control platform for the consolidation of multiple industrial workloads to achieve real-time performance~\cite{intelwhitepaper}.
GE’s Automation and Controls platform provides industrial software, control systems and embedded computing platforms to optimize our customers’ assets and equipment~\cite{gewhitepaper}. The platform combines what was formerly known as GE Intelligent Platforms and Alstom’s Power Automation \& Controls~\cite{wiki:geintell}.
Omneo, the big data analytic platform in Siemens, is a platform that converts fragmented, error-filled data from across the value chain into actionable product performance intelligence~\cite{siemens}.

However, few detailed information on the architecture, implementation and performance of these systems are shown in white papers the companies provide. In this paper, we will show all the design details and evaluation result on each component in our system as an anchor for people's reference.
The following of this section will summarize and compare the lower level components and techniques needed and their features. We will first introduce some works on the messaging protocol to collect the data. Then, the messaging systems used to partition and distribute the data streams are discussed. Next, we will introduce NoSQL databases to store these data and last, we will describe computation frameworks and systems where the data can be processed.

\subsection{Messaging protocols \& messaging systems}
With the growth number of data sources and data volume, messaging protocols and systems designed particular for IoT gain its popularity. Distributed messaging systems and messaging protocols are always implemented together to achieve high data velocity and system scalability.
\subsubsection{Messaging protocols}
In this paper, we consider four of the most common and popular TCP/IP based messaging protocols and provide a summary of each: MQTT, CoAP, STOMP and AMQP. All of these protocols are built intended for resource constrained devices and networks, thus they can be efficiently implemented especially on wireless embedded systems using batteries.

MQ telemetry transport, first developed by IBM in 1999 and known as MQTT, is a machine-to-machine (M2M) IoT connectivity protocol~\cite{mqtt}.
The 'MQ' in 'MQTT' came from IBM's MQ message queuing product line.
MQTT enables the publish-subscribe mode and provides many-to-many broadcast capabilities.
Although light weight is a common feature in all IoT messaging protocols, MQTT is extremely light weight that it has only five methods. This design works perfectly on small, low power devices, in the other hand, the lack of functionality in MQTT may not satisfy larger system's requirements.

Another widely used system is Advanced Message Queuing Protocol (AMQP).
AMQP is an open internet protocol for reliably sending and receiving messages~\cite{vinoski2006advanced} originated in 2003 by John O'Hara at JPMorgan Chase in London, UK~\cite{o2007toward}.
AMQP makes it possible for everyone to build a diverse, coherent messaging ecosystem capable for a wide range of features related to messaging, including reliable queuing, topic-based publish/subscribe messagging, flexible routing, transactions and security~\cite{qpid2013open,amqpvmware}.

The Constrained Application Protocol (CoAP) is a specialized web transfer protocol intended for use with resource-constrained nodes and networks that need to be controlled or supervised remotely.
CoAP packets are much smaller than HTTP TCP flows for saving space.
Unlike MQTT, CoAP is primarily a one-to-one protocol for transferring state information between client and server~\cite{mqttcoapIoT}.

STOMP (Simple/Streaming Text Oriented Messaging Protocol) is text-based, analogous to HTTP in terms of how it looks under the covers. Like AMQP, STOMP provides a message (or frame) header with properties, and a frame body. The design principles here were to create something simple, and widely-interoperable~\cite{amqpvmware}.

\eat{DDS,JMS}

\subsubsection{Messaging system}
In order to partition, separate the data streams among the cluster and use messages asynchronously, most of the messaging systems are carefully designed with features like reliability, clustering, multi-protocol, multi-language supporting and scalability.
These systems such as ActiveMQ, RabbitMQ, ZeroMQ, Apache Qpid, Kafka, IronMQ share similarities. A white paper ~\cite{braveNewGeek} shows some useful throughput and latency benchmarks for readers' reference.

Unlike a messaging system, no message broker are needed in the implementation of ZeroMQ and this leads to a higher throughput and lower latency than they other systems. The drawbacks of such design is also explicit: though ZeroMQ guarantees that messages will be delivered atomically intact and ordered but does not guarantee the delivery of them.

RabbitMQ is one of the open source softwares that supports several messing protocols including AMQP, STOMP, MQTT and HTTP through the use of plugins. RabbitMQ supports both persistent and non-persistent delivery. To guarantee delivery, these brokers use message acknowledgements which also incurs a massive latency penalty~\cite{braveNewGeek}.

Kafka is a distributed messaging system for collecting and delivering high volumes of log data with low latency~\cite{kreps2011kafka}. Also, it is suitable for both offline and online message consumption. High availability and horizontally scaling are also other key features of Kafka through the use of ZooKeeper.

\subsection{NoSQL databases}
Data storage is a critical component of our system. Traditional relational databases are widely used in the past decades, but it is not suitable ~\cite{madden2012databases} for large amount of time series data without explicit structures and relations. In order to fully use the large amount of data, a variety of NoSQL databases are proposed and developed including key-value stores, document stores and wide column stores~\cite{khazaei2015choose}.

\subsubsection{Key-value stores}
Key-value stores use a map or dictionary as a collection of key-value pairs as the fundamental data model.
Berkeley DB (BDB)~\cite{olson1999berkeley} as an example of key-value stores is a software library that provides a high-performance embedded database for key/value data.
Based on Berkeley DB many other key-value stores are designed and developed such as Oracle NoSQL Database~\cite{joshi2012oracle} and Project Voldemort~\cite{feinberg2011project}.
Oracle NoSQL Database~\cite{joshi2012oracle} provides major and minor keys, flexible durability and consistency policies, and integration with both MapReduce infrastructure and conventional relational data.

HBase is an open source, non-relational, distributed database modeled after Google's BigTable~\cite{chang2008bigtable} and written in Java. It is developed as part of Apache Software Foundation's Apache Hadoop project and runs on top of HDFS (Hadoop Distributed Filesystem), providing BigTable-like capabilities for Hadoop~\cite{wiki:hbase}.
Apache Cassandra, initially created by Facebook, is an open source distributed database management system designed to handle large amounts of data across many commodity servers, providing high availability with no single point of failure~\cite{wiki:cassandra}. Cassandra also offers support for MapReduce, Apache Pig and Apache Hive. Besides, CQL(Cassandra Query Language), a SQL-like alternative to the traditional RPC interface is also provided.

\subsubsection{Document stores}
Document stores differ on the definition of "document" but generally, they all all assume that documents encapsulate and encode data in some standard formats or encodings including XML, YAML, and JSON.
Apache CouchDB, commonly referred to as CouchDB, is an open source database that focuses on ease of use~\cite{wiki:couchDB}, especially for Web. It uses JSON for documents, JavaScript for MapReduce indexes, and regular HTTP for its API~\cite{web:couchDB}.
Couchbase Server is a open source, distributed(shared-nothing architecture), multi-model NoSQL database engineered for performance, scalability, and availability, optimized for interactive applications~\cite{wiki:couchbase}. It enables developers to build applications easier and faster by leveraging the power of SQL with the flexibility of JSON~\cite{web:couchbase}.
MongoDB is a cross-platform document-oriented database. Classified as a NoSQL database, MongoDB eschews the traditional table-based relational database structure in favor of JSON-like documents with dynamic schemas (MongoDB calls the format BSON), making the integration of data in certain types of applications easier and faster~\cite{wiki:mongoDB}.

As we get time series data from sensors and simulators continuously, we choose to use HBase because we need key based access to data when storing or retrieving and SQL is not needed when we query data.

\subsection{Computation frameworks and systems}
MapReduce, Storm and Spark are three most widely used computation models, while they have different use cases. This subsection shows the features of each one of them.
\subsubsection{MapReduce}
MapReduce is a programming model and an associated implementation for processing and generating large data sets with a parallel, distributed algorithm on a cluster. Conceptually similar approaches have been very well known since 1995 with the Message Passing Interface standard having reduce and scatter operations. MapReduce libraries have been written in many programming languages, with different levels of optimization. A popular open-source implementation that has support for distributed shuffles is part of Apache Hadoop. The name MapReduce originally referred to the proprietary Google technology, but has since been genericized~\cite{dean2008mapreduce}.
\subsubsection{Storm}
Apache Storm is a distributed computation framework written predominantly in the Clojure programming language. Originally created by Nathan Marz and team at BackType, the project was open sourced after being acquired by Twitter~\cite{toshniwal2014storm}.
\subsubsection{Spark}
Apache Spark is an open source cluster computing framework originally developed in the AMPLab at University of California, Berkeley but was later donated to the Apache Software Foundation where it remains today. In contrast to Hadoop's two-stage disk-based MapReduce paradigm, Spark's multi-stage in-memory primitives provides performance up to 100 times faster for certain applications. By allowing user programs to load data into a cluster's memory and query it repeatedly, Spark is well-suited to machine learning algorithms~\cite{engle2012shark}.

An online report~\cite{StormSparkCompare} provides and detailed overview and effective comparison of the internals of both the Storm and Spark streaming platforms. Overall design and architecture are also covered in this report. Some of the differences are briefly are listed here. Storm and spark are implemented in JVM based languages: Clojure and Scala, respectively. Storm supports strictly streaming processing while user can customize it to be micro-batching. Spark provides micro-batching internally while Spark streaming is a wrapper over its micro-batching framework. In some older version, Storm uses ZeroMQ as in its messaging layer, but it now moves to Netty. Spark uses a combination of Netty and Akka.

